Weakly Durable High-Performance Transactions

Existing disk-based database systems largely fall into two categories -- they either provide very high performance but few guarantees, or expose the transaction abstraction satisfying the full ACID guarantees at the cost of lower performance. In this paper, we present an alternative that achieves the best of both worlds, namely good performance and transactional properties. Our key observation is that, because of the frequent use of synchronization primitives, systems with strong durability can hardly utilize the extremely high parallelism granted by modern storage devices. Thus, we explore the notion of weakly durable transactions, and discuss how to safely relax durability without compromising other transactional properties. We present AciKV, a transactional system whose design is centered around weak durability. AciKV exposes to users the normal transactional interface, but what sets it apart from others is a new "persist" primitive that decouples durability from commit. AciKV is a middle ground between systems that perform fast atomic operations, and ones that support transactions; this middle ground is useful as it provides similar performance to the former, while prevents isolation and consistency anomalies like the latter. Our evaluation using the YCSB benchmark shows that AciKV, under workloads that involve write requests, exhibits more than two orders of magnitude higher throughput than existing strongly durable systems.

==> code/client-round.py.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k}{def} \PY{n+nf}{client\PYZus{}round}\PY{p}{(}\PY{n+nb}{round}\PY{p}{,} \PY{n}{onion\PYZus{}keys}\PY{p}{,} \PY{n}{buddy}\PY{p}{)}\PY{p}{:}
  \PY{c+c1}{\PYZsh{}\PYZsh{}\PYZsh{} \textbf{Phase 1:} Circuit Setup}
  \PY{n}{onion1}\PY{p}{,} \PY{n}{circuit1} \PY{o}{=} \PY{n}{rand\PYZus{}circuit}\PY{p}{(}\PY{n+nb}{round}\PY{p}{,} \PY{n}{onion\PYZus{}keys}\PY{p}{)}
  \PY{n}{onion2}\PY{p}{,} \PY{n}{circuit2} \PY{o}{=} \PY{n}{rand\PYZus{}circuit}\PY{p}{(}\PY{n+nb}{round}\PY{p}{,} \PY{n}{onion\PYZus{}keys}\PY{p}{)}

  \PY{n}{receipts} \PY{o}{=} \PY{n}{send\PYZus{}setup\PYZus{}onions}\PY{p}{(}\PY{p}{[}\PY{n}{onion1}\PY{p}{,} \PY{n}{onion2}\PY{p}{]}\PY{p}{)}
  \PY{n}{h1} \PY{o}{=} \PY{n}{onion\PYZus{}decrypt\PYZus{}aes}\PY{p}{(}\PY{n}{circuit1}\PY{o}{.}\PY{n}{keys}\PY{p}{,} \PY{n}{receipts}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}\PY{p}{)}
  \PY{n}{h2} \PY{o}{=} \PY{n}{onion\PYZus{}decrypt\PYZus{}aes}\PY{p}{(}\PY{n}{circuit2}\PY{o}{.}\PY{n}{keys}\PY{p}{,} \PY{n}{receipts}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}\PY{p}{)}
  \PY{k}{if} \PY{n}{h1} \PY{o}{!=} \PY{n+nb}{hash}\PY{p}{(}\PY{n}{circuit1}\PY{o}{.}\PY{n}{endpoint}\PY{p}{)} \PY{o+ow}{or}
     \PY{n}{h2} \PY{o}{!=} \PY{n+nb}{hash}\PY{p}{(}\PY{n}{circuit2}\PY{o}{.}\PY{n}{endpoint}\PY{p}{)}\PY{p}{:}
    \PY{k}{raise} \PY{n+ne}{Exception}\PY{p}{(}\PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{hash mismatch; aborting round}\PY{l+s+s2}{\PYZdq{}}\PY{p}{)}

  \PY{c+c1}{\PYZsh{}\PYZsh{}\PYZsh{} \textbf{Phase 2:} Noise Verification}
  \PY{n}{counts}\PY{p}{,} \PY{n}{sigs} \PY{o}{=} \PY{n}{recv\PYZus{}noise\PYZus{}signatures}\PY{p}{(}\PY{p}{)}
  \PY{n}{noise} \PY{o}{=} \PY{l+m+mi}{0}
  \PY{k}{for} \PY{n}{i} \PY{o+ow}{in} \PY{n+nb}{range}\PY{p}{(}\PY{n}{servers}\PY{p}{)}\PY{p}{:}
    \PY{k}{if} \PY{n}{verify}\PY{p}{(}\PY{n}{sigs}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{p}{,} \PY{n}{servers}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{o}{.}\PY{n}{signing\PYZus{}key}\PY{p}{)}\PY{p}{:}
      \PY{n}{noise} \PY{o}{+}\PY{o}{=} \PY{n}{counts}\PY{p}{[}\PY{n}{i}\PY{p}{]}
  \PY{k}{if} \PY{n}{noise} \PY{o}{\PYZlt{}} \PY{n}{required\PYZus{}noise}\PY{p}{:}
    \PY{k}{raise} \PY{n+ne}{Exception}\PY{p}{(}\PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{insufficient noise present}\PY{l+s+s2}{\PYZdq{}}\PY{p}{)}

  \PY{c+c1}{\PYZsh{}\PYZsh{}\PYZsh{} \textbf{Phase 3:} Circuit Exchange}
  \PY{n}{buddy\PYZus{}endpoint} \PY{o}{=} \PY{n}{exchange\PYZus{}circuit}\PY{p}{(}\PY{n}{buddy}\PY{p}{,} \PY{n}{circuit1}\PY{o}{.}\PY{n}{endpoint}\PY{p}{)}
  \PY{k}{if} \PY{n}{buddy\PYZus{}endpoint} \PY{o+ow}{is} \PY{k+kc}{None}\PY{p}{:}
    \PY{n}{buddy} \PY{o}{=} \PY{n+nb+bp}{self}
    \PY{n}{buddy\PYZus{}endpoint} \PY{o}{=} \PY{n}{circuit2}\PY{o}{.}\PY{n}{endpoint}

  \PY{n}{conn} \PY{o}{=} \PY{n}{connect\PYZus{}circuit}\PY{p}{(}\PY{n}{buddy\PYZus{}endpoint}\PY{p}{)}

  \PY{c+c1}{\PYZsh{}\PYZsh{}\PYZsh{} \textbf{Phase 4:} Circuit Messaging}
  \PY{k}{def} \PY{n+nf}{read\PYZus{}loop}\PY{p}{(}\PY{p}{)}\PY{p}{:}
    \PY{k}{while} \PY{n}{data} \PY{p}{:}\PY{o}{=} \PY{n}{conn}\PY{o}{.}\PY{n}{read}\PY{p}{(}\PY{p}{)}\PY{p}{:}
      \PY{c+c1}{\PYZsh{} Note: don't need to onion\_decrypt\_aes here.}
      \PY{n}{msg} \PY{o}{=} \PY{n}{decrypt\PYZus{}aes}\PY{p}{(}\PY{n}{buddy}\PY{o}{.}\PY{n}{secret}\PY{p}{,} \PY{n}{data}\PY{p}{)}
      \PY{n}{play\PYZus{}voice\PYZus{}packet}\PY{p}{(}\PY{n}{msg}\PY{p}{)}
  \PY{n}{spawn\PYZus{}thread}\PY{p}{(}\PY{n}{read\PYZus{}loop}\PY{p}{)}

  \PY{k}{while} \PY{n}{r} \PY{p}{:}\PY{o}{=} \PY{n}{recv\PYZus{}subround\PYZus{}announcement}\PY{p}{(}\PY{p}{)}\PY{p}{:}
    \PY{n}{msg} \PY{o}{=} \PY{n}{encrypt\PYZus{}aes}\PY{p}{(}\PY{n}{buddy}\PY{o}{.}\PY{n}{secret}\PY{p}{,} \PY{n}{get\PYZus{}voice\PYZus{}packet}\PY{p}{(}\PY{p}{)}\PY{p}{)}
    \PY{n}{onion} \PY{o}{=} \PY{n}{onion\PYZus{}encrypt\PYZus{}aes}\PY{p}{(}\PY{n}{circuit1}\PY{o}{.}\PY{n}{keys}\PY{p}{,} \PY{n}{msg}\PY{p}{)}
    \PY{n}{send\PYZus{}voice\PYZus{}onion}\PY{p}{(}\PY{n}{r}\PY{o}{.}\PY{n}{subround}\PY{p}{,} \PY{n}{onion}\PY{p}{)}
\end{Verbatim}


==> code/fmt.tex <==

\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@si\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.44,0.63,0.82}{##1}}}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.44,0.13}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.25,0.63,0.44}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.38,0.63,0.69}{##1}}}
\expandafter\def\csname PY@tok@mb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.25,0.63,0.44}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.44,0.63}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.44,0.13}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.32,0.47,0.09}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.25,0.44,0.63}{##1}}}
\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.44,0.13}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.44,0.13}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.25,0.44,0.63}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.25,0.44,0.63}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.14,0.33,0.53}{##1}}}
\expandafter\def\csname PY@tok@ch\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.38,0.63,0.69}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.38,0.63,0.69}{##1}}\def\PY@bc##1{\setlength{\fboxsep}{0pt}\colorbox[rgb]{1.00,0.94,0.94}{\strut ##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.44,0.13}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.44,0.13}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.44,0.13}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.25,0.44,0.63}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.25,0.63,0.44}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.38,0.68,0.84}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.38,0.84}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.44,0.13}{##1}}}
\expandafter\def\csname PY@tok@cpf\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.38,0.63,0.69}{##1}}}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.25,0.44,0.63}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.25,0.63,0.44}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.38,0.84}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.84,0.33,0.22}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.44,0.13}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.44,0.13}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@nd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.33,0.33,0.33}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.13,0.44}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.25,0.63,0.44}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.38,0.63,0.69}{##1}}}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.78,0.36,0.04}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.05,0.52,0.71}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.25,0.44,0.63}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.44,0.13}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.56,0.13,0.00}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.02,0.16,0.45}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.38,0.84}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.25,0.44,0.63}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.25,0.44,0.63}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.02,0.16,0.49}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.38,0.63,0.69}{##1}}}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.38,0.84}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.78,0.36,0.04}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.05,0.52,0.71}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother



==> data.tex <==
% Macros for data points we use throughout the paper.
\newcommand{\overallLatency}{$\SI{990}{\milli\second}$\xspace}

% Some of these values are duplicated in the Makefile.


==> hdr.tex <==
\input{rev}

\usepackage{fancyhdr}
\pagestyle{fancy}
\fancyhf{}
\renewcommand{\headrulewidth}{0pt}
\lhead{Rev.~\therev}
\rhead{\thedate}
\cfoot{\thepage}


==> impl.tex <==
\section{Implementation}
\label{sec:impl}

The \sys prototype is around $6{,}500$ lines of C code and is available at link suppressed for anonymity.



==> limitations.tex <==
\section{Limitations}
\label{s:limitations}

Being upfront about \sys's limitations is important.
These could be problems for future work.


==> overview.tex <==
\section{Overview}
\label{s:overview}



\autoref{fig:overview} shows how users communicate through \sys at a high level.
Now we will explain it.

\subsection{Goals and threat model}
\label{s:goals}

\paragraph{Security goal.}

\paragraph{Threat model.}



==> rev.tex <==
\gdef\therev{9b6218d}
\gdef\thedate{2021-05-08 02:08:12 +0800}

